Recent Results From BaBar in Tau Physics

The BaBar collaboration has accumulated over 400 million tau-pairs which can be used to study charged leptonic and hadronic weak currents to unprecedented precision. This note presents results on lepton universality, measurements of |V_us|, and searches for tau decays which violate lepton flavour conservation, or tau decays that proceed through a suppressed second class current.

==> Introduction.tex <==

%\chapter{Introduction}
\pagenumbering{arabic}

\section{Introduction}


The BaBar collaboration has accumulated over 400 million $\tau$-pairs. Using this large data sample it is possible to test charged leptonic and hadronic weak currents to unprcedented precision. Of particular interest are topics in lepton universality where the relative weak coupling strength of the different generations of leptons is tested, measuring $\Vus$ using hadronic $\tau$ decays and comparing the measured values with unitarity predictions from the cabbibo kobayashim meskawa (CKM) matrix, searches for $\tau $ decays in which the lepton number at the vertices is not conserved, and searches for $\tau$ decays that proceed through a suppressed second class current. 





==> TitlePage.tex <==
\begin{titlepage}
\begin{flushleft}
\mbox{\normalsize {\babar\ }Analysis Document \#XXXX, Version 001} \\
\end{flushleft}
\vskip 20pt

\begin{center}
{\large\bf 
Recent Results In $\tau$ Physics From BaBar \\
}
\end{center}

\begin{center} 
M.J.~Lewczuk  \\
University of Victoria
\end{center} 


 
\begin{abstract}
This note presents a study of the  
\end{abstract}
\end{titlepage}

